Long-time asymptotics of the Navier-Stokes and vorticity equations on R^3

We use the vorticity formulation to study the long-time behavior of solutions to the Navier-Stokes equation on R^3. We assume that the initial vorticity is small and decays algebraically at infinity. After introducing self-similar variables, we compute the long-time asymptotics of the rescaled vorticity equation up to second order. Each term in the asymptotics is a self-similar divergence-free vector field with Gaussian decay at infinity, and the coefficients in the expansion can be determined by solving a finite system of ordinary differential equations. As a consequence of our results, we are able to characterize the set of solutions for which the velocity field converges to zero faster than t^(-5/4) in energy norm. In particular, we show that these solutions lie on a smooth invariant submanifold of codimension 11 in our function space.

==> Fig1.tex <==
% height 5.5 cm
% width 11.0 cm	
\smash{\hbox{
\point	9.10	3.00 	{$\Re(\lambda)$}
\point	8.00	5.00 	{$\Im(\lambda)$}
\point	5.20	4.50 	{$\textstyle \frac{m}{2}-\frac{1}{4}$}
\point	4.10	2.20 	{$\textstyle -\frac{3}{2}$}
\point	5.20	2.20 	{$-1$}
\point	1.50	1.50 	{$\sigma_c(\Lambda)$}
}}



==> Fig2.tex <==
% height 6.0 cm
% width 9.0 cm	
\smash{\hbox{
\point	7.20	0.50 	{$\cW_2$}
\point -0.50	3.60 	{$\cV$}
\point	6.00	5.30 	{$W_s^{loc}$}
}}


